Delta Denoising Score

We introduce Delta Denoising Score (DDS), a novel scoring function for text-based image editing that guides minimal modifications of an input image towards the content described in a target prompt. DDS leverages the rich generative prior of text-to-image diffusion models and can be used as a loss term in an optimization problem to steer an image towards a desired direction dictated by a text. DDS utilizes the Score Distillation Sampling (SDS) mechanism for the purpose of image editing. We show that using only SDS often produces non-detailed and blurry outputs due to noisy gradients. To address this issue, DDS uses a prompt that matches the input image to identify and remove undesired erroneous directions of SDS. Our key premise is that SDS should be zero when calculated on pairs of matched prompts and images, meaning that if the score is non-zero, its gradients can be attributed to the erroneous component of SDS. Our analysis demonstrates the competence of DDS for text based image-to-image translation. We further show that DDS can be used to train an effective zero-shot image translation model. Experimental results indicate that DDS outperforms existing methods in terms of stability and quality, highlighting its potential for real-world applications in text-based image editing.

==> 05_limitation.tex <==
\input{figures/tex_limitation}
\section{Limitations}

Our \ourmethod{} works well for in distilling text-driven image-to-image translations. However, there are cases that the results are imperfect due to the inherent limitation of the text-to-image model, in particular its language model. A noticeable problem is the binding of adjectives to the nouns. A typical example is demonstrated in Figure \ref{fig:limietaion}(top), where the orange color is not well bind to the curtains, and thus licks to the entire bedroom. Another example, displayed in the bottom row, where the dog's reflection is replaced with a shadow and caused unwanted changes in the background details.

We also acknowledge that the multi-task model can be better trained and may be further improved by combining multiple experts training \cite{balaji2022eDiff}, which uses multiple network, or utilize subset of paired data and train our network under semi-supervised settings.


==> figures/table_zero_shot.tex <==
\begin{table}
\caption{\bf{Quantitative results for zero shot text driven image editing.} \it{We evaluate our method using InstructPix2Pix synthetic dataset.}}
 \footnotesize
 \centering
%  \vspace{0.2cm}
\begin{tabular}{lcc}
\toprule
& CLIP score $\uparrow$ &  LPIPS $\downarrow$ \\
\midrule
SDEdit &  &  \\
Prompt2Prompt &  $0.33 \pm  0.03$ &  $0.38 \pm 0.17 $\\
Ours &  &   \\
\bottomrule
\end{tabular}
\label{tab:images}
\end{table}




==> figures/tex_supp_net_result_figures.tex <==
\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{figures/supp_net_result_figures1.pdf}
    \caption{\bf{Unsupervised image-to-image translation-- characters.} {\it Different networks were trained to change the person in the image to various characters.
    The networks were trained on FFHQ in-the-wild dataset (unaligned) \cite{karras2019style} and tested on images from COCO dataset \cite{caesar2018coco}.}}
    \label{fig:supp_characters1}
\end{figure*}

